Growth Tight Actions

We introduce and systematically study the concept of a growth tight action. This generalizes growth tightness for word metrics as initiated by Grigorchuk and de la Harpe. Given a finitely generated, non-elementary group $G$ acting on a $G$--space $\mathcal{X}$, we prove that if $G$ contains a strongly contracting element and if $G$ is not too badly distorted in $\mathcal{X}$, then the action of $G$ on $\mathcal{X}$ is a growth tight action. It follows that if $\mathcal{X}$ is a cocompact, relatively hyperbolic $G$--space, then the action of $G$ on $\mathcal{X}$ is a growth tight action. This generalizes all previously known results for growth tightness of cocompact actions: every already known example of a group that admits a growth tight action and has some infinite, infinite index normal subgroups is relatively hyperbolic, and, conversely, relatively hyperbolic groups admit growth tight actions. This also allows us to prove that many CAT(0) groups, including flip-graph-manifold groups and many Right Angled Artin Groups, and snowflake groups admit cocompact, growth tight actions. These provide first examples of non-relatively hyperbolic groups admitting interesting growth tight actions. Our main result applies as well to cusp uniform actions on hyperbolic spaces and to the action of the mapping class group on Teichmueller space with the Teichmueller metric. Towards the proof of our main result, we give equivalent characterizations of strongly contracting elements and produce new examples of group actions with strongly contracting elements.

==> embedding.tex <==


\endinput
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "Main"
%%% End: 


==> rank1.tex <==
In this section we relate path system projections to rank 1 isometries.


\begin{definition}\label{def:ballcontracting}
  $\pi\from \X\to \A$ is $(C,D,E)$--\emph{contracting} if $d(x_0,x_1)<\frac{1}{E}d(x_0,\A)-D$ implies
  $d(\pi(x_0),\pi(x_1))\leqslant C$.
We say $\pi$ is
\emph{strongly contracting} if it is $(C,D,1)$--contracting for some
$C,\,D\geqslant 0$.
\end{definition}


Some remarks are in order concerning overuse of the term `contracting'.
The term `stongly contracting' is not standard.
Indeed, in most of the literature what we are calling `strongly contracting' is just called `contracting'.
This is the case, for example, in the literature on rank 1 isometries of CAT(0) spaces.
However, Masur and Minsky \cite{MasMin99} use `contracting' in the sense of \fullref{def:ballcontracting}, as do subsequent papers on the geometry of the mappping class group.
In the present paper, we choose the term `strongly contracting' to emphasize that we want $E=1$.

Recall that in \fullref{part:gt} we also have Sisto's $\ps$--contracting and related definitions of contracting and strongly contracting elements.
For a $\ps$--contracting element $h$, \fullref{lemmaprojection} tells us that there is a $\ps$--contracting projection to an axis of $h$.
We will see in \fullref{lemma:Sistoprojectionproperties} that this projection is contracting.
Similarly, we will see in
\fullref{proposition:almostminimizingstronglycontracting} that an
element $h$ is strongly contracting in the sense of
\fullref{def:stronglycontracting} if and only if closest point
projection to the axis of $h$ is coarsely well defined and strongly
contracting in the sense of \fullref{def:ballcontracting}.




\begin{lemma}[{cf. \cite[Lemma~2.4]{Sis11}}]\label{lemma:Sistoprojectionproperties}
  Let $\ps$ be a path system.
Let $\pi\from \X\to \A$ be a $C$--$\ps$--contracting projection.
Suppose there exists a $(\lambda,\epsilon)$--quasi-geodesic connecting
$x$ to $y$ in $\ps$, then there is a constant $D$ depending on
$\lambda$, $\epsilon$, and $C$ such that:
\begin{enumerate}
\item (coarse Lipschitz) $d(\pi(x),\pi(y))\leqslant \lambda
  d(x,y)+D$.\label{item:coarselipschitz} %D=\left(\lambda\epsilon(\lambda+2)+4C\right)
\item (contracting) If
  $d(x,y)<\frac{1}{\lambda}d(x,\A)-D$
  then $d(\pi(x),\pi(y))\leqslant C$.\label{item:contracting} %D=\left(3\frac{C}{\lambda}+\epsilon(\lambda+2)\right)
\end{enumerate}
Suppose there exists a $(\lambda,\epsilon)$--quasi-geodesic connecting
$x$ to $\pi(x)$ in $\ps$, then there is a constant $D$ depending on
$\lambda$, $\epsilon$, and $C$ such that:
\begin{enumerate}
\setcounter{enumi}{2}
\item (closest point projection) $d(x,\pi(x))\leqslant \lambda
  d(x,\A)+D$.\label{item:closestpointprojection} %D=\left(\lambda\epsilon(\lambda+1)+C\right)
\end{enumerate}
\end{lemma}
\fullref{lemma:Sistoprojectionproperties} is just a restatement of 
\cite[Lemma~2.4]{Sis11}, without uniformizing the constants. 
The proofs are identical.


\begin{lemma}\label{corollary:strongcontracting}
  If $\pi\from \X\to\A$ is a $\ps$--contracting projection and $\ps$ is
  minimizing then $\pi$ is strongly contracting and 
coarsely agrees with
  closest point projection to $\A$.
\end{lemma}
\begin{proof}
Strong contraction comes from
\fullref{lemma:Sistoprojectionproperties} (\ref{item:contracting}), since
we can take each $\lambda=1$.

Let $x\in\X$ and let $a\in\A$ such that $d(x,\A)=d(x,a)$.
Suppose that $d(\pi(x),a)>2C$.
Let $\path\in\ps$ be a geodesic from $x$ to $a$.
Since $d(a,\pi(a))\leqslant C$, we have $d(\pi(x),\pi(a))>C$, so $\path$
enters $\clnbhd{C}{\pi(x)}$.
Thus:
\[d(x,a)\geqslant d(x,\pi(x))+d(\pi(x),a)-2C>d(x,\pi(x))\]
This contradicts the choice of $a$.
\end{proof}


\begin{proposition}\label{proposition:almostminimizingstronglycontracting}
  $\pi\from \X\to \A$.
The following are equivalent:
\begin{enumerate}
\item $\pi$ is a contracting projection for the path system of all geodesics.\label{item:almostgeodesicprojecction}
\item $\pi$ is a $\ps$--contracting projection for some minimizing path
  system $\ps$.\label{item:almostminimizing}
\item $\pi$ is strongly contracting and coarsely agrees with closest
  point projection to $\A$.\label{item:stronglycontracting}
\item $\pi$ has the Bounded Geodesic Image Property and coarsely
  agrees with closest
  point projection to $\A$.\label{item:boundedgeodesicimage}
\end{enumerate}
\end{proposition}
\begin{proof}
(\ref{item:almostgeodesicprojecction})$\implies$(\ref{item:almostminimizing}) is clear.
(\ref{item:almostminimizing})$\implies$(\ref{item:stronglycontracting})
is \fullref{corollary:strongcontracting}.
(\ref{item:stronglycontracting}) and (\ref{item:boundedgeodesicimage})
are equivalent by \fullref{lemma:boundedgeodesicimage}.
We need only show (\ref{item:boundedgeodesicimage})$\implies$(\ref{item:almostgeodesicprojecction}).

Assume (\ref{item:boundedgeodesicimage}), so $\pi\from \X\to \A$ is a map such that:
  \begin{itemize}
  \item $d(x,\pi(x))\leqslant d(x,\A)+C$ for all $x\in \X$, and
\item for every geodesic $\gamma$ if $\gamma\cap\clnbhd{D}{\A}=\emptyset$
  then $\diam(\pi(\gamma))\leqslant C$.
  \end{itemize}
Let $\ps$ be the path system consisting of all geodesics.
Let $\gamma\from [0,T]\to X$ be a geodesic with projection larger
than $C$.
Let $t_0$ and $t_1$ be the first and last times,
respectively, such that $\gamma_t\in {N_{D}(\A)}$.
Then: \[d(\pi(\gamma_0),\gamma_{t_0})\leqslant
d(\pi(\gamma_0),\pi(\gamma_{t_0}))+d(\pi(\gamma_{t_0}),\gamma_{t_0})\leqslant 2C+D\]
Similarly, $d(\pi(\gamma_T),\gamma_{t_1})\leqslant 2C+D$.
Thus, $\pi$ is a $(2C+D)$--$\ps$--contraction.
This completes the proof of \fullref{proposition:almostminimizingstronglycontracting}.
\end{proof}


\endinput

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "Main"
%%% End: 

